Multidisciplinary Design Optimization Approach to Integrated Space Mission Planning and Spacecraft Design

Space mission planning and spacecraft design are tightly coupled and need to be considered together for optimal performance; however, this integrated optimization problem results in a large-scale Mixed-Integer Nonlinear Programming (MINLP) problem, which is challenging to solve. In response to this challenge, this paper proposes a new solution approach to this MINLP problem by iterative solving a set of coupled subproblems via the augmented Lagrangian coordination approach following the philosophy of Multi-disciplinary Design Optimization (MDO). The proposed approach leverages the unique structure of the problem that enables its decomposition into a set of coupled subproblems of different types: a Mixed-Integer Quadratic Programming (MIQP) subproblem for mission planning and one or more Nonlinear Programming (NLP) subproblem(s) for spacecraft design. Since specialized MIQP or NLP solvers can be applied to each subproblem, the proposed approach can efficiently solve the otherwise intractable integrated MINLP problem. An automatic and effective method to find an initial solution for this iterative approach is also proposed so that the optimization can be performed without the need for a user-defined initial guess. In the demonstration case study, a human lunar exploration mission sequence is optimized with a subsystem-level parametric spacecraft design model. Compared to the state-of-the-art method, the proposed formulation can obtain a better solution with a shorter computational time even without parallelization. For larger problems, the proposed solution approach can also be easily parallelizable and thus is expected to be further advantageous and scalable.

==> Ascend 2021 Journal Revision (1)/Eqns/MissionParameter.tex <==
\begin{table}
\caption{\label{MisisonParameter} Variables and parameters used in the space transportation scheduling problem}
\centering
\begin{tabular}{p{0.5\textwidth}p{0.15\textwidth}}
\hline Parameters & Assumption \\\hline

Spacecraft Propellant type, $zeta$ & LH2/LOx \\
Propellant $I_{sp}$, s & 420 \\
Type of Spacecraft designed  & 1 \\
Number of vehicles for each type & 6 \\
Crew mass (including space suit), kg/person & 100 \\
Crew consumption, kg/day/person & 8.655 \\
Spacecraft maintenance, structure mass/flight & 1\% \\
ISRU maintenance rate, system mass/ year & 5\% \\

\hline
\end{tabular}
\end{table}

==> Ascend 2021 Journal Revision (1)/Eqns/ProbDef.tex <==
\begin{equation}
\label{SL_obj}
\min \quad \mathcal{J}=\sum_{t\in \mathcal{T}} \sum_{(v,i,j)\in \mathcal{A}} (\boldsymbol{a}_{vijt}^{T} \boldsymbol{x}_{vijt} + {a'}_{vijt}^{T} m_{d_{v}} u_{vijt})
\end{equation}

subject to
\begin{equation}
\label{SL_constr1}
\sum_{(v,j):(v,i,j)\in \mathcal{A}} \left[\begin{array}{c}
\boldsymbol{x}_{vijt} \\
m_{d_v}u_{vijt}
\end{array}\right] - \sum_{(v,j):(v,i,j)\in \mathcal{A}} Q_{vjit} \left[\begin{array}{c}
\boldsymbol{x}_{vji(t-\Delta t_{ji})} \\
m_{d_{v}} u_{vji(t-\Delta t_{ji})}
\end{array}\right]
\leq \boldsymbol{d}_{it} \quad \forall t\in \mathcal{T}\quad \forall i\in \mathcal{N} 
\end{equation}


\begin{equation}
\label{SL_constr2}
    {H}_{vij} \boldsymbol{x}_{vijt} \leq \boldsymbol{e}_v u_{vijt}  \quad \forall t\in \mathcal{T} \quad \forall (v,i,j)\in \mathcal{A}
\end{equation}

\begin{equation}
\label{SL_constr3}
\left\{\begin{array}{ll}
\boldsymbol{x}_{vijt} \geq \boldsymbol{0}_{p \times 1}  &\text { if } t \in W_{i j} \\
\boldsymbol{x}_{vijt} =\boldsymbol{0}_{p \times 1} \quad &\text { otherwise }
\end{array} \quad \forall(v, i, j) \in \mathcal{A}\quad \forall t\in \mathcal{T}\right.
\end{equation}

\begin{equation}
\label{SL_vehicle_sizing}
    m_{d_v} = \mathcal{F}(\boldsymbol{e}_v, \zeta_v)  \quad \forall v\in \mathcal{V} 
\end{equation}

\begin{equation}
\label{xdef}
\begin{aligned}
\boldsymbol{x}_{v i j t}=\left[\begin{array}{c}
x_{1} \\
x_{2} \\
\vdots \\
x_{p}
\end{array}\right]_{v i j t}, \quad \begin{aligned}
&x_{n} \in \mathbb{R}_{\geq 0} \quad \forall n \in \mathcal{C}_{c} \\
&x_{n} \in \mathbb{Z}_{\geq 0} \quad \forall n \in \mathcal{C}_{d}
\end{aligned} \quad \forall(v, i, j, t) \in \mathcal{A} \\
\end{aligned}
\end{equation}

\begin{equation}
\label{udef}
{u}_{v i j t} \in \mathbb{Z}_{\geq 0}  \quad \forall(v, i, j, t) \in \mathcal{A} 
\end{equation}

\begin{equation}
\label{evdef}
\boldsymbol{e}_v =  \left[\begin{array}{c}
m_{p} \\
m_{f} 
\end{array}\right]_{v}, \quad m_{p_v}, m_{f_v}, m_{d_v} \in \mathbb{R}_{\geq 0}, \quad \forall v \in \mathcal{V} 
\end{equation}

==> Ascend 2021 Journal Revision (1)/Eqns/Subprob1_Def.tex <==
\begin{equation}
\label{SubSL_obj}
\min \quad \sum_{t\in \mathcal{T}} \sum_{(v,i,j)\in \mathcal{A}} (\boldsymbol{a}_{vijt}^{T} \boldsymbol{x}_{vijt} + {a'}_{vijt}^{T} m_{d_{v}} u_{vijt}) + \phi_{1}\left(\boldsymbol{c}_{1}\left(\boldsymbol{y}, \boldsymbol{y}_{1}\right)\right) 
\end{equation}

subject to
\begin{equation}
\label{SubSL_constr1}
\sum_{(v,j):(v,i,j)\in \mathcal{A}} \left[\begin{array}{c}
\boldsymbol{x}_{vijt} \\
m_{d_v}u_{vijt}
\end{array}\right] - \sum_{(v,j):(v,i,j)\in \mathcal{A}} Q_{vjit} \left[\begin{array}{c}
\boldsymbol{x}_{vji(t-\Delta t_{ji})} \\
m_{d_{v}} u_{vji(t-\Delta t_{ji})}
\end{array}\right]
\leq \boldsymbol{d}_{it} \quad \forall t\in \mathcal{T}\quad \forall i\in \mathcal{N} 
\end{equation}


\begin{equation}
\label{SubSL_constr2}
    {H}_{vij} \boldsymbol{x}_{vijt} \leq \boldsymbol{e}_v u_{vijt}  \quad \forall t\in \mathcal{T} \quad \forall (v,i,j)\in \mathcal{A}
\end{equation}

\begin{equation}
\left\{\begin{array}{ll}
\boldsymbol{x}_{vijt} \geq \boldsymbol{0}_{p \times 1}  &\text { if } t \in W_{i j} \\
\boldsymbol{x}_{vijt} =\boldsymbol{0}_{p \times 1} \quad &\text { otherwise }
\end{array} \quad \forall(v, i, j, t) \in \mathcal{A}\right.
\end{equation}

\begin{equation}
\begin{aligned}
\boldsymbol{x}_{v i j t}=\left[\begin{array}{c}
x_{1} \\
x_{2} \\
\vdots \\
x_{p}
\end{array}\right]_{v i j t}, \quad \begin{aligned}
&x_{n} \in \mathbb{R}_{\geq 0} \quad \forall n \in \mathcal{C}_{c} \\
&x_{n} \in \mathbb{Z}_{\geq 0} \quad \forall n \in \mathcal{C}_{d}
\end{aligned} \quad \forall(v, i, j, t) \in \mathcal{A} \\
\end{aligned}
\end{equation}

\begin{equation}
{u}_{v i j t} \in \mathbb{Z}_{\geq 0}  \quad \forall(v, i, j, t) \in \mathcal{A} 
\end{equation}

\begin{equation}
\boldsymbol{e}_v =  \left[\begin{array}{c}
m_{p} \\
m_{f} 
\end{array}\right]_{v}, \quad m_{p_v}, m_{f_v}, m_{d_v} \in \mathbb{R}_{\geq 0}, \quad \forall v \in \mathcal{V} 
\end{equation}

\begin{equation}
\boldsymbol{y}_1 = [m_{p_1}, m_{f_1}, m_{d_1}, \dots, m_{p_N}, m_{f_N}, m_{d_N}]
\end{equation}

==> Ascend 2021 Journal Revision (1)/Tables/10gen.tex <==
\begin{table}[!t]
\centering
\caption{\label{10gen}Instance 1 results comparison with different PWL increments at 10 generations}
\begin{tabular}{ccccc} 
\hline\hline
PWL increment, kg       & Algorithm & Average opt. time, s & Best IMLEO, kg & Worst IMLEO, kg  \\ 
\hline
\multirow{4}{*}{10,000} & ACO       & 66.93        & 707,882        & 724,776          \\
                        & GA        & 72.81        & 684,755        & 724,776          \\
                        & PSO       & 69.06        & 696,625        & 724,776          \\
                        & Proposed  & 20.02        & 724,776        & -                \\ 
\hline
\multirow{4}{*}{5,000}  & ACO       & 65.99        & 694,224        & 694,224          \\
                        & GA        & 71.27        & 681,842        & 694,224          \\
                        & PSO       & 67.98        & 694,224        & 694,224          \\
                        & Proposed  & 13.47        & 694,224        & -                \\ 
\hline
\multirow{4}{*}{2,500}  & ACO       & 72.27        & 705,550        & infeasible       \\
                        & GA        & 80.58        & 759,326        & infeasible       \\
                        & PSO       & 74.57        & 700,227        & infeasible       \\
                        & Proposed  & 11.98        & 676,862        & -                \\ 
\hline
\multirow{4}{*}{1,250}  & ACO       & 65.93        & 677,303        & 677,303          \\
                        & GA        & 70.16        & 677,303        & 677,303          \\
                        & PSO       & 69.00        & 677,303        & 677,303          \\
                        & Proposed  & 13.83        & 677,204        & -                \\ 
\hline
\multirow{4}{*}{625}    & ACO       & 67.21        & 677,283        & 677,283          \\
                        & GA        & 69.42        & 677,283        & 677,283          \\
                        & PSO       & 68.33        & 677,283        & 677,283          \\
                        & Proposed  & 13.18        & 677,072        & -                \\
\hline\hline
\end{tabular}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/ACOall.tex <==
\begin{table}[hbt!]
\centering
\caption{\label{ACOall}ACO embedded optimization results with 2,500 kg PWL increment}
\begin{tabular}{ccccc} 
\hline\hline
Instance & Number of generations & Optimization time, s & \multicolumn{1}{l}{Best IMLEO, kg} & \multicolumn{1}{l}{Worst IMLEO, kg}  \\ 
\hline
         & 10                    & 72.27                & 705,550                            & infeasible                                  \\
1        & 50                    & 360.9                & 705,550                            & 830,350                              \\
         & 100                   & 721.2                & 685,146                            & 783,343                              \\ 
\hline
         & 10                    & 91.37                & 461,323                            & 831,125                              \\
2        & 50                    & 452.4                & 420,662                            & 631,469                              \\
         & 100                   & 904.0                & 420,662                            & 541,799                              \\ 
\hline
         & 10                    & 147.0                & 460,524                            & infeasible                                  \\
3        & 50                    & 732.0                & 459,157                            & 565,537                              \\
         & 100                   & 1466                 & 426,322                            & 508,066                              \\ 
\hline
         & 10                    & 80.68                & 470,538                            & 470,538                              \\
4        & 50                    & 403.6                & 470,538                            & 470,538                              \\
         & 100                   & 804.6                & 470,538                            & 470,538                              \\ 
\hline
         & 10                    & 74.45                & 454,849                            & 484,095                              \\
5        & 50                    & 371.3                & 453,073                            & 466,563                              \\
         & 100                   & 740.9                & 445,776                            & 461,279                              \\ 
\hline
         & 10                    & 95.43                & 321,152                            & 359,303                              \\
6        & 50                    & 476.7                & 299,690                            & 336,976                              \\
         & 100                   & 952.5                & 299,690                            & 330,914                              \\ 
\hline
         & 10                    & 171.8                & 323,436                            & 348,874                              \\
7        & 50                    & 858.8                & 315,515                            & 326,136                              \\
         & 100                   & 1716                 & 313,764                            & 323,436                              \\ 
\hline
         & 10                    & 94.14                & 375,746                            & 425,749                              \\
8        & 50                    & 468.6                & 359,239                            & 401,878                              \\
         & 100                   & 934.7                & 351,292                            & 394,226                              \\
\hline\hline
\end{tabular}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/ALCdefault.tex <==
\begin{table}[!htbp]
\centering
\caption{\label{ALCdefault}Instance 1 optimization results by the proposed decomposition-based formulation}
\begin{tabular}{ccccclcc} 
\hline\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}PWL\\increment, kg\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}PWL~ \\mesh points\end{tabular}} & \multicolumn{3}{c}{Optimization time, s}                             &                      & \multicolumn{2}{c}{IMLEO, kg}                \\ 
\cline{3-5}\cline{7-8}
                                                                            &                                                                             & PLW-based            & Decomposition-based        & \multirow{2}{*}{Total} & \multicolumn{1}{c}{} & PWL-based            & Final                 \\
                                                                            &                                                                             & initial solution     & iterations         &                        & \multicolumn{1}{c}{} & initial solution     & solution              \\ 
\hline
10,000                                                                      & 13                                                                          & 3.461                & 20.02                & 23.48                  &                      & 741,115              & 724,776               \\
5,000                                                                       & 36                                                                          & 4.769                & 13.47                & 18.24                  &                      & 700,684              & 694,224               \\
2,500                                                                       & 120                                                                         & 4.754                & 11.98                & 16.73                  &                      & 677,035              & 676,862               \\
1,250                                                                       & 425                                                                         & 28.09                & 13.83                & 41.92                  &                      & 677,343              & 677,204               \\
625                                                                         & 1,595                                                                       & 465.5                & 13.18                & 478.7                  &                      & 677,315              & 677,072               \\ 
\hline\hline
\multicolumn{1}{l}{}                                                        & \multicolumn{1}{l}{}                                                        & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}   &                      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} 
\end{tabular}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/ALCinstances.tex <==
\begin{table}[!htbp]
\centering
\caption{\label{ALCinstances}Decomposition-based optimization results with 2,500 kg increment for all instances}
\begin{tabular}{cccclcc} 
\hline\hline
            & \multicolumn{3}{c}{Optimization time, s}                        &                      & \multicolumn{2}{c}{IMLEO, kg}  \\ 
\cline{2-4}\cline{6-7}
Instance    & PWL-based        & Decomposition-based & \multirow{2}{*}{Total} & \multicolumn{1}{c}{} & PWL-based        & Final       \\
            & initial solution & iterations        &                        & \multicolumn{1}{c}{} & initial solution & solution    \\ 
\hline
1 (default) & 4.754            & 11.98               & 16.73                  &                      & 677,035          & 676,862     \\
2           & 38.66            & 10.70               & 49.35                  &                      & 401,191          & 401,093     \\
3           & 38.66            & 61.57               & 100.2                  &                      & 386,257          & 387,535     \\
4           & 10.53            & 22.63               & 33.16                  &                      & 470,788          & 470,406     \\
5           & 75.35            & 94.06               & 154.7                  &                      & 442,596          & 442,605     \\
6           & 24.09            & 14.30               & 38.39                  &                      & 293,095          & 293,095     \\
7           & 100.1            & 44.02               & 144.1                  &                      & 286,154          & 302,041     \\
8           & 31.50            & 14.47               & 45.97                  &                      & 344,397          & 344,423     \\
\hline\hline
\end{tabular}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/CaseList.tex <==
\begin{table}[hbt!]
\caption{\label{CaseList} Case study instances specifications}
\centering
\begin{tabular}{ccccc} 
\hline\hline
Instance index & \begin{tabular}[c]{@{}c@{}}Type(s) of SC\\ ~desinged\end{tabular} & \begin{tabular}[c]{@{}c@{}}Number of SC\\ per type\end{tabular} & SC sizing model & Mission payload  \\ 
\hline
1 (default)              & 1                                                                 & 6                                                               & conservative    & default          \\
2              & 2                                                                 & 3                                                               & conservative    & default          \\
3              & 6                                                                 & 1                                                               & conservative    & default          \\
4              & 2                                                                 & 3                                                               & conservative    & increased        \\
5              & 1                                                                 & 6                                                               & aggressive      & default          \\
6              & 2                                                                 & 3                                                               & aggressive      & default          \\
7              & 6                                                                 & 1                                                               & aggressive      & default          \\
8              & 2                                                                 & 3                                                               & aggressive      & increased        \\
\hline\hline
\end{tabular}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/GAall.tex <==
\begin{table}[hbt!]
\centering
\caption{\label{GAall}GA embedded optimization results with 2,500 kg PWL increment}
\begin{tabular}{ccccc} 
\hline\hline
Instance & Number of generations & Optimization time, s & \multicolumn{1}{l}{Best IMLEO, kg} & \multicolumn{1}{l}{Worst IMLEO, kg}  \\ 
\hline
         & 10                    & 80.58                & 759,326                            & infeasible                                  \\
1        & 50                    & 413.1                & 712,515                            & infeasible                                  \\
         & 100                   & 814.8                & 712,515                            & infeasible                                  \\ 
\hline
         & 10                    & 98.80                & 437,974                            & infeasible                                  \\
2        & 50                    & 511.9                & 437,275                            & infeasible                                  \\
         & 100                   & 1010                 & 414,034                            & infeasible                                  \\ 
\hline
         & 10                    & 158.7                & 427,682                            & infeasible                                  \\
3        & 50                    & 840.4                & 419,610                            & infeasible                                  \\
         & 100                   & 1686                 & 398,507                            & infeasible                                  \\ 
\hline
         & 10                    & 85.71                & 470,538                            & 470,538                              \\
4        & 50                    & 434.4                & 470,538                            & 470,538                              \\
         & 100                   & 872.8                & 470,538                            & 470,538                              \\ 
\hline
         & 10                    & 84.28                & 455,676                            & 484,630                              \\
5        & 50                    & 406.7                & 455,676                            & 479,622                              \\
         & 100                   & 806.1                & 455,676                            & 476,852                              \\ 
\hline
         & 10                    & 106.2                & 306,077                            & 359,839                              \\
6        & 50                    & 512.0                & 297,363                            & 329,513                              \\
         & 100                   & 1020                 & 297,183                            & 316,152                              \\ 
\hline
         & 10                    & 178.5                & 304,792                            & 345,599                              \\
7        & 50                    & 866.8                & 296,631                            & 323,739                              \\
         & 100                   & 1708                 & 291,836                            & 305,488                              \\ 
\hline
         & 10                    & 111.7                & 358,082                            & 513,027                              \\
8        & 50                    & 518.8                & 353,113                            & 388,664                              \\
         & 100                   & 998.2                & 349,502                            & 371,646                              \\
\hline\hline
\end{tabular}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/LunarMissionDemand.tex <==
\begin{table}[h]
\caption{\label{LunarMissionDemand} Lunar campaign commodity demand and supply}
\centering
\begin{tabular}{cccc}
\hline\hline Payload Type & Node & Date & Supply/Demand (increased instance) \\\hline
\multicolumn{4}{c}{Outbound to the Moon} \\\hline
Crew & Earth & 0, 365 & 4 \\
Habitat, Equipment, and Propellant, kg & Earth & 0, 365 & $\infty$ \\
Crew & Moon & 5, 370 & -4 \\
Habitat \& Equipment, kg & Moon & 5, 370 & -2000 (-3000)\\

\hline\multicolumn{4}{c}{Inbound to the Earth} \\\hline
Crew & Moon & 8, 373 & 4\\
Returned mass, kg & Moon & 8, 373 & 1000 (1500)\\
Crew & Earth & 13, 378 & -4 \\
Returned mass, kg & Earth & 13, 378 & -1000 (-1500)\\

\hline\hline
\end{tabular}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/MissionParameter.tex <==
\begin{table}[h]
\caption{\label{MisisonParameter} Parameters used in the default instance (Instance 1) of the case study}
\centering
\begin{tabular}{p{0.5\textwidth}p{0.15\textwidth}}
\hline\hline Parameters & Assumed values \\\hline

Spacecraft Propellant type & LH2/LOX \\
Propellant $I_{sp}$, s & 420 \\
Propellant density $\rho_f$, kg/m\textsuperscript{3} & 360\\
Spacecraft miscellaneous mass fraction $c_{misc}$ (see Eq.~\eqref{sizing}) & 0.05\\
Spacecraft payload capacity range, kg & [500, 10000]\\
Spacecraft propellant capacity range, kg & [1000, 100000]\\
Type(s) of spacecraft designed  & 1 \\
Number of vehicles for each type & 6 \\
Crew mass (including space suit), kg/person & 100 \\
Crew consumption, kg/day/person & 8.655 \\
Spacecraft maintenance, structure mass/flight & 1\% \\

\hline\hline
\end{tabular}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/Old&Unused/ALCresults2.tex <==
\begin{table}[h]
\caption{\label{ALCresults2} Optimization results by the decomposition-based formulation, set 2}
\centering
\begin{tabular}{cccccc}
\hline\hline
Piecewise linear   approximation step size, kg & 8000   & 4000   & 2000   & 1000   & 500    \\
\hline
Initial guess IMLEO, kg                        & 700103 & 688884 & 678633 & 677737 & 677390 \\
IMLEO, kg                                      & 694820 & 686199 & 678391 & 677542 & 677245 \\
$m_p$, kg                                         & 2882   & 2860   & 2838   & 2836   & 2834   \\
$m_f$, kg                                         & 44335  & 43627  & 42980  & 42923  & 42901  \\
$m_d$, kg                                         & 13098  & 12919  & 12757  & 12743  & 12736  \\
\hline
Initial guess generation time, s               & 5.176  & 12.19  & 3.569  & 33.22  & 1070   \\
Decomposition-based optimization time, s       & 24.23  & 19.75  & 13.30  & 13.36  & 13.97  \\
Total optimization time, s                     & 29.40  & 31.95  & 16.87  & 46.58  & 1084  \\
\hline\hline
\end{tabular}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/Old&Unused/CombinedBestResults.tex <==
\begin{table}[h]
\caption{\label{CombBestRes} Best-/Worst-Case results comparison} 
\centering
\begin{tabular}{ccccc}
\hline\hline
            & \multicolumn{1}{c}{\multirow{2}{*}{Proposed formulation}} & \multicolumn{3}{c}{Embedded optimization method} \\
            \cline{3-5}
            & \multicolumn{1}{c}{}                            & Ant Colony & GA     & PSO    \\
            \hline
Best IMLEO, kg   & 676930                                          & 681302     & 728831 & 677221 \\
Optimization time, s & 16.27                                           & 45.77      & 836.6  & 793.9 \\
            \hline
Worst IMLEO, kg   & 727558                                          & inf     & inf & inf \\
Optimization time, s & 33.96                                           & 45.77      & 836.6  & 793.9 \\
\hline\hline
\end{tabular}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/Old&Unused/PSOincrements.tex <==
\begin{table}
\centering
\caption{\label{PSOincrements}\new{Default instance PSO embedded optimization results with various increments}}
\begin{tabular}{cccc} 
\hline\hline
PWL increment, kg   & Algorithm & Opt.
  time, s & IMLEO, kg  \\ 
\hline
\multirow{2}{*}{10,000} & PSO       & 69.06           & 719,166    \\
                        & Proposed  & 20.02           & 724,776    \\ 
\hline
\multirow{2}{*}{5,000}  & PSO       & 67.98           & 694,224    \\
                        & Proposed  & 13.47           & 694,224    \\ 
\hline
\multirow{2}{*}{2,500}  & PSO       & 68.22           & 764,402    \\
                        & Proposed  & 10.36           & 676,862    \\ 
\hline
\multirow{2}{*}{1,250}  & PSO       & 69.00           & 677,303    \\
                        & Proposed  & 13.83           & 677,204    \\ 
\hline
\multirow{2}{*}{625}    & PSO       & 68.33           & 677,283    \\
                        & Proposed  & 13.18           & 677,072    \\
\hline\hline
\end{tabular}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/Old&Unused/PSOinstances10gen.tex <==
\begin{table}
\centering
\caption{\label{PSOinstances10gen}\new{PSO embedded optimization results for all instances at 10 generations}}
\begin{tabular}{cccccc} 
\hline\hline
Instance           & Algorithm & Opt. time, s & Avg. IMLEO, kg & Best IMLEO, kg & Worst IMLEO, kg  \\ 
\hline
\multirow{2}{*}{1 (default)} & PSO       & 74.57        & 755,394        & 700,227        & inf              \\
                   & Proposed  & 11.98        & 676,862        & -              & -                \\ 
\hline
\multirow{2}{*}{2} & PSO       & 84.70        & 472,243        & 436,363        & inf              \\
                   & Proposed  & 10.70        & 401,093        & -              & -                \\ 
\hline
\multirow{2}{*}{3} & PSO       & 153.0        & 453,084        & 423,873        & inf              \\
                   & Proposed  & 61.57        & 387,535        & -              & -                \\ 
\hline
\multirow{2}{*}{4} & PSO       & 82.52        & 470,538        & 470,538        & 470,538          \\
                   & Proposed  & 22.63        & 470,406        & -              & -                \\ 
\hline
\multirow{2}{*}{5} & PSO       & 75.36        & 460,932        & 451,269        & 470,869          \\
                   & Proposed  & 94.06        & 442,605        & -              & -                \\ 
\hline
\multirow{2}{*}{6} & PSO       & 96.64        & 320,680        & 305,457        & 337,105          \\
                   & Proposed  & 14.30        & 293,095        & -              & -                \\ 
\hline
\multirow{2}{*}{7} & PSO       & 172.3        & 322,115        & 302,791        & 358,768          \\
                   & Proposed  & 44.02        & 302,041        & -              & -                \\ 
\hline
\multirow{2}{*}{8} & PSO       & 94.21        & 372,485        & 355,767        & 395,748          \\
                   & Proposed  & 14.47        & 344,423        & -              & -                \\
\hline\hline
\end{tabular}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/Old&Unused/basecase_comparison.tex <==
\begin{table}
\caption{\label{BasecaseComparison} \textcolor{red}{Default instance average results by the embedded optimization over 10 iterations}}
\centering
\begin{tabular}{cccc}
\hline\hline
Algorithm & Number of generations & Optimization time, s & IMLEO, kg  \\ 
\hline
          & 10                    & 72.27                & 782,304    \\
ACO       & 50                    & 360.9                & 742,573    \\
          & 100                   & 721.2                & 718,586    \\ 
\hline
          & 10                    & 80.58                & 822,926    \\
GA        & 50                    & 413.1                & 770,917    \\
          & 100                   & 814.8                & 752,836    \\ 
\hline
          & 10                    & 74.57                & 755,394    \\
PSO       & 50                    & 381.7                & 702,581    \\
          & 100                   & 765.3                & 691,196    \\ 
\hline
Proposed  & -                   & 10.36                & 676,862    \\
\hline\hline
\end{tabular}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/Old&Unused/embedded_highlight.tex <==
\begin{table}[h]
\caption{\label{EmbeddedHighlight} Results of the state-of-the-art embedded optimization}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccccc}
\hline\hline
% \multicolumn{1}{c}{Algorithm} & \multicolumn{1}{c}{Number of generations} & Optimization Time, s & Best IMLEO, kg  \\
% \hline
% \multirow{3}{*}{Ant Colony Optimization}    
%      & 10  & 85.03    & 723090 \\
%      & 50   & 391.7    & 747398 \\
%      & 100 & 776.0      & 689287 \\
% \hline
% \multirow{3}{*}{Genetic Algorithm}           
%      & 10  & 86.18    & 764301 \\
%      & 50  & 413.6    & 746702 \\
%      & 100 & 836.6    & 728831 \\
% \hline
% \multirow{3}{*}{Particle Swarm Optimization} 
%      & 10 & 84.69    & inf    \\                              
%      & 50  & 397.9    & 677659 \\
%      & 100 & 793.9    & 677221 \\ 
%      \hline\hline
     
     
     
\multicolumn{1}{c}{Algorithm} & \multicolumn{3}{c}{Ant Colony Optimization} & \multicolumn{3}{c}{Genetic Algorithm} & \multicolumn{3}{c}{Particle Swarm Optimization} \\
\hline
Number of generations & 10 & 50 & 100 & 10 & 50 & 100 & 10 & 50 & 100 \\
Best Solution IMLEO, kg  & 723,090  & 747,398& 689,287 & 764,301& 746,702 & 728,831 & inf & 677,659& 677,221\\
Optimization Time, s &85.03& 391.7  & 776.0  & 86.18 & 413.6 & 836.6 & 84.69 & 397.9 & 793.9\\
\hline\hline 
\end{tabular}}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/Old&Unused/embedded_highlight2.tex <==
\begin{table}[h]
\caption{\label{EmbeddedFullTable2} Summary of the embedded optimization results}
\centering
\centering
\resizebox{0.75\textwidth}{!}{%
\begin{tabular}{cccc}
\hline\hline
\multicolumn{1}{c}{Algorithm}                        & \multicolumn{1}{l}{Number of generations} & Optimization time, s & IMLEO, kg  \\
\hline
\multirow{15}{*}{Ant Colony Optimization}    
     & \multirow{3}{*}{5}                                    & 45.35    & 820891 \\
     &                                                       & 45.06    & inf    \\
     &                                                       & 45.77    & 681302 \\
     \cline{2-4}
     & \multirow{3}{*}{10}                                     & 83.19    & 806153 \\
     &                                                     & 85.03    & 723090 \\
     &                                                      & 83.81    & 793031 \\\cline{2-4}
     & \multirow{3}{*}{20}                                       & 161.4    & 714202 \\
     &                                                           & 161.2    & 801618 \\
     &                                                           & 162.3    & 710166 \\\cline{2-4}
     & \multirow{3}{*}{50}                                      & 389.8    & 761514 \\
     &                                                          & 391.2    & 765182 \\
     &                                                          & 391.7    & 747398 \\\cline{2-4}
     & \multirow{3}{*}{100}                                    & 776.0      & 689287 \\
     &                                                          & 771.9    & 732297 \\
     &                                                        & 775.9    & 691874 \\
\hline
\multirow{15}{*}{Genetic Algorithm}           
     & \multirow{3}{*}{5}                                      & 46.50     & inf    \\
     &                                                         & 45.71    & inf    \\
     &                                                        & 46.09    & inf    \\\cline{2-4}
     & \multirow{3}{*}{10}                                     & 85.38    & inf    \\
     &                                                      & 86.18    & 764301 \\
     &                                                      & 83.97    & inf    \\\cline{2-4}
     & \multirow{3}{*}{20}                                   & 161.9    & inf    \\
     &                                                        & 172.4    & 761116 \\
     &                                                       & 161.7    & inf    \\\cline{2-4}
     & \multirow{3}{*}{50}                                    & 394.7    & inf    \\
     &                                                       & 413.6    & 746702 \\
     &                                                          & 394.6    & inf    \\\cline{2-4}
     & \multirow{3}{*}{100}                                   & 836.6    & 728831 \\
     &                                                        & 788.3    & 875069 \\
     &                                                         & 777.7    & inf    \\
\hline
\multirow{15}{*}{Particle Swarm Optimization} 
     & \multirow{3}{*}{5}                                      & 46.54    & inf    \\
     &                                                         & 46.57    & inf    \\
     &                                                       & 46.26    & 711382 \\\cline{2-4}
     & \multirow{3}{*}{10}                                    & 84.75    & inf    \\
     &                                                        & 84.69    & inf    \\
     &                                                       & 85.22    & inf    \\\cline{2-4}
     & \multirow{3}{*}{20}                                     & 162.5    & 726951 \\
     &                                                       & 162.1    & 688182 \\
     &                                                         & 161.6    & inf    \\\cline{2-4}
     & \multirow{3}{*}{50}                                     & 392.3    & inf    \\
     &                                                       & 397.9    & 677659 \\
     &                                                         & 394.6    & 714169 \\\cline{2-4}
     & \multirow{3}{*}{100}                                   & 788.9    & 677754 \\
     &                                                         & 793.9    & 677221 \\
     &                                                        & 791.2    & 677316 \\
     \hline\hline
\end{tabular}}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/Old&Unused/heuristics_results.tex <==
\begin{table}[h]
\caption{\label{EmbeddedFullTable} Summary of the embedded optimization results}
\centering
\resizebox{0.67\textwidth}{!}{%
\begin{tabular}{ccccc}
\hline\hline
\multicolumn{1}{c}{Algorithm}                        & \multicolumn{1}{l}{Number of Generations} & Iteration Number & Run Time, s & IMLEO, kg  \\
\hline
\multirow{15}{*}{Ant Colony Optimization}    & \multirow{3}{*}{5}                        & 1                & 45.35    & 820891 \\
                                                     &                                           & 2                & 45.06    & inf    \\
                                                     &                                           & 3                & 45.77    & 681302 \\
                                                     \cline{2-5}
                                                     & \multirow{3}{*}{10}                       & 1                & 83.19    & 806153 \\
                                                     &                                           & 2                & 85.03    & 723090 \\
                                                     &                                           & 3                & 83.81    & 793031 \\\cline{2-5}
                                                     & \multirow{3}{*}{20}                       & 1                & 161.4    & 714202 \\
                                                     &                                           & 2                & 161.2    & 801618 \\
                                                     &                                           & 3                & 162.3    & 710166 \\\cline{2-5}
                                                     & \multirow{3}{*}{50}                       & 1                & 389.8    & 761514 \\
                                                     &                                           & 2                & 391.2    & 765182 \\
                                                     &                                           & 3                & 391.7    & 747398 \\\cline{2-5}
                                                     & \multirow{3}{*}{100}                      & 1                & 776.0      & 689287 \\
                                                     &                                           & 2                & 771.9    & 732297 \\
                                                     &                                           & 3                & 775.9    & 691874 \\
\hline
\multirow{15}{*}{Genetic Algorithm}           & \multirow{3}{*}{5}                        & 1                & 46.50     & inf    \\
                                                     &                                           & 2                & 45.71    & inf    \\
                                                     &                                           & 3                & 46.09    & inf    \\\cline{2-5}
                                                     & \multirow{3}{*}{10}                       & 1                & 85.38    & inf    \\
                                                     &                                           & 2                & 86.18    & 764301 \\
                                                     &                                           & 3                & 83.97    & inf    \\\cline{2-5}
                                                     & \multirow{3}{*}{20}                       & 1                & 161.9    & inf    \\
                                                     &                                           & 2                & 172.4    & 761116 \\
                                                     &                                           & 3                & 161.7    & inf    \\\cline{2-5}
                                                     & \multirow{3}{*}{50}                       & 1                & 394.7    & inf    \\
                                                     &                                           & 2                & 413.6    & 746702 \\
                                                     &                                           & 3                & 394.6    & inf    \\\cline{2-5}
                                                     & \multirow{3}{*}{100}                      & 1                & 836.6    & 728831 \\
                                                     &                                           & 2                & 788.3    & 875069 \\
                                                     &                                           & 3                & 777.7    & inf    \\
\hline
\multirow{15}{*}{Particle Swarm Optimization} & \multirow{3}{*}{5}                        & 1                & 46.54    & inf    \\
                                                     &                                           & 2                & 46.57    & inf    \\
                                                     &                                           & 3                & 46.26    & 711382 \\\cline{2-5}
                                                     & \multirow{3}{*}{10}                       & 1                & 84.75    & inf    \\
                                                     &                                           & 2                & 84.69    & inf    \\
                                                     &                                           & 3                & 85.22    & inf    \\\cline{2-5}
                                                     & \multirow{3}{*}{20}                       & 1                & 162.5    & 726951 \\
                                                     &                                           & 2                & 162.1    & 688182 \\
                                                     &                                           & 3                & 161.6    & inf    \\\cline{2-5}
                                                     & \multirow{3}{*}{50}                       & 1                & 392.3    & inf    \\
                                                     &                                           & 2                & 397.9    & 677659 \\
                                                     &                                           & 3                & 394.6    & 714169 \\\cline{2-5}
                                                     & \multirow{3}{*}{100}                      & 1                & 788.9    & 677754 \\
                                                     &                                           & 2                & 793.9    & 677221 \\
                                                     &                                           & 3                & 791.2    & 677316\\\hline\hline
\end{tabular}}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/PSOall.tex <==
\begin{table}[!htbp]
\centering
\caption{\label{PSOall}PSO embedded optimization results with 2,500 kg PWL increment}
\begin{tabular}{ccccc}
\hline\hline
Instance & Number of generations & Optimization time, s & \multicolumn{1}{l}{Best IMLEO, kg} & \multicolumn{1}{l}{Worst IMLEO, kg}  \\ 
\hline
         & 10                    & 74.57                & 700,227                            & infeasible                                  \\
1        & 50                    & 381.7                & 680,234                            & 731,419                              \\
         & 100                   & 765.3                & 680,234                            & 710,650                              \\ 
\hline
         & 10                    & 84.70                & 436,363                            & infeasible                                  \\
2        & 50                    & 440.0                & 403,448                            & 439,154                              \\
         & 100                   & 881.6                & 402,976                            & 412,622                              \\ 
\hline
         & 10                    & 153.0                & 423,873                            & infeasible                                  \\
3        & 50                    & 794.1                & 421,689                            & 436,608                              \\
         & 100                   & 1620                 & 408,388                            & 421,829                              \\ 
\hline
         & 10                    & 82.52                & 470,538                            & 470,538                              \\
4        & 50                    & 419.9                & 470,538                            & 470,538                              \\
         & 100                   & 842.3                & 470,538                            & 470,538                              \\ 
\hline
         & 10                    & 75.36                & 451,269                            & 470,869                              \\
5        & 50                    & 373.9                & 445,230                            & 458,624                              \\
         & 100                   & 748.6                & 445,230                            & 450,841                              \\ 
\hline
         & 10                    & 96.64                & 305,457                            & 337,105                              \\
6        & 50                    & 476.7                & 301,583                            & 314,667                              \\
         & 100                   & 949.7                & 298,414                            & 306,893                              \\ 
\hline
         & 10                    & 172.3                & 302,791                            & 358,768                              \\
7        & 50                    & 881.8                & 298,361                            & 313,493                              \\
         & 100                   & 1772                 & 298,361                            & 310,755                              \\ 
\hline
         & 10                    & 94.21                & 355,767                            & 395,748                              \\
8        & 50                    & 466.1                & 350,294                            & 363,609                              \\
         & 100                   & 934.3                & 348,585                            & 359,040                              \\
\hline\hline
\end{tabular}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/PSOinstances.tex <==
\begin{table}[!b]
\centering
\caption{\label{PSOinstances}PSO embedded opt. results comparison: 2,500 kg PWL increment, all instances, 10 and 100 generations}
\begin{tabular}{cccccc} 
\hline\hline
Instance                     & Algorithm            & Number of generations & Average opt. time, s & Best IMLEO, kg & Worst IMLEO, kg  \\ 
\hline
\multirow{3}{*}{1 (default)} & \multirow{2}{*}{PSO} & 10                    & 74.57        & 700,227        & infeasible       \\
                             &                      & 100                   & 765.3        & 680,234        & 710,650          \\
                             & Proposed             & -                     & 11.98        & 676,862        & -                \\ 
\hline
\multirow{3}{*}{2}           & \multirow{2}{*}{PSO} & 10                    & 84.70        & 436,363        & infeasible       \\
                             &                      & 100                   & 881.6        & 402,976        & 412,622          \\
                             & Proposed             & -                     & 10.70        & 401,093        & -                \\ 
\hline
\multirow{3}{*}{3}           & \multirow{2}{*}{PSO} & 10                    & 153.0        & 423,873        & infeasible       \\
                             &                      & 100                   & 1620         & 408,388        & 421,829          \\
                             & Proposed             & -                     & 61.57        & 387,535        & -                \\ 
\hline
\multirow{3}{*}{4}           & \multirow{2}{*}{PSO} & 10                    & 82.52        & 470,538        & 470,538          \\
                             &                      & 100                   & 842.3        & 470,538        & 470,538          \\
                             & Proposed             & -                     & 22.63        & 470,406        & -                \\ 
\hline
\multirow{3}{*}{5}           & \multirow{2}{*}{PSO} & 10                    & 75.36        & 451,269        & 470,869          \\
                             &                      & 100                   & 748.6        & 445,230        & 450,841          \\
                             & Proposed             & -                     & 94.06        & 442,605        & -                \\ 
\hline
\multirow{3}{*}{6}           & \multirow{2}{*}{PSO} & 10                    & 96.64        & 305,457        & 337,105          \\
                             &                      & 100                   & 949.7        & 298,414        & 306,893          \\
                             & Proposed             & -                     & 14.30        & 293,095        & -                \\ 
\hline
\multirow{3}{*}{7}           & \multirow{2}{*}{PSO} & 10                    & 172.3        & 302,791        & 358,768          \\
                             &                      & 100                   & 1772         & 298,361        & 310,755          \\
                             & Proposed             & -                     & 44.02        & 302,041        & -                \\ 
\hline
\multirow{3}{*}{8}           & \multirow{2}{*}{PSO} & 10                    & 94.21        & 355,767        & 395,748          \\
                             &                      & 100                   & 934.3        & 348,585        & 359,040          \\
                             & Proposed             & -                     & 14.47        & 344,423        & -                \\
\hline\hline
\end{tabular}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/ProbDef_var_list.tex <==
\begin{table}[h]
\caption{\label{tab_SLvar} Variables and parameters used in the space transportation scheduling problem}
\centering
\begin{tabular}{ll}
\hline\hline Name & 
\begin{tabular}{p{0.7\textwidth}}Description\end{tabular} \\\hline

{\emph{Variables} }&\\

\hline
$\boldsymbol{x}_{vijt}$ & 
\begin{tabular}{p{0.7\textwidth}}
Commodity flow variable, or the quantity of the commodity delivered from node $i$ to $j$ at time $t$ by spacecraft $v$. $\boldsymbol{x}_{vijt} \geq 0$. Each component of this variable can contain either continuous variables ($\mathcal{C}_{c}$) or discrete variables ($\mathcal{C}_{d}$). This vector will be $\mathbb{R}^p$ if the total commodity variation is $p$. 
\end{tabular} \\

$u_{vijt}$ & 
\begin{tabular}{p{0.7\textwidth}}
Spacecraft flow variable, which indicates the number of spacecraft type $v$ moving from node $i$ to $j$ at time $t$ ($\in \mathbb{R}$). This variable is integer scalar. 
\end{tabular} \\

$\boldsymbol{e}_v$ & 
\begin{tabular}{p{0.7\textwidth}}
Spacecraft design variables and parameters. In this problem, it includes payload capacity $m_p$ and propellant capacity $m_f$ ($\in \mathbb{R}^2$).
\end{tabular}\\

$m_{d_v}$ & 
\begin{tabular}{p{0.7\textwidth}}
Dry mass of spacecraft $v$ ($\in \mathbb{R}$).
\end{tabular}\\

\hline
{\emph{Parameters}} &\\

\hline
$\boldsymbol{a}_{vijt}$ & 
\begin{tabular}{p{0.7\textwidth}}
Cost coefficient of commodity ($\in \mathbb{R}^p$).
\end{tabular}\\

${a'}_{vijt}$ & 
\begin{tabular}{p{0.7\textwidth}}
Cost coefficient of spacecraft ($\in \mathbb{R}$). 
\end{tabular}\\

$\boldsymbol{d}_{it}$ & 
\begin{tabular}{p{0.7\textwidth}}
Demands/supplies of different commodities and spacecraft at node $i$ at time $t$ ($\in \mathbb{R}^{p+1}$).
\end{tabular}\\

$Q_{vijt}$ & 
\begin{tabular}{p{0.7\textwidth}}
Transformation matrix ($\in\R^{(p+1)\times(p+1)}$).
\end{tabular}\\


$H_{vij}$ & 
\begin{tabular}{p{0.7\textwidth}}
Concurrency constraint matrix ($\in \R^{2\times p}$).
\end{tabular}\\

$W_{ij}$ & 
\begin{tabular}{p{0.7\textwidth}}
Launch window vector, which indicates the available launch window of spacecraft.
\end{tabular}\\

$\mathcal{F}(-)$ & 
\begin{tabular}{p{0.7\textwidth}}
Spacecraft sizing function. This illustrates the nonlinear relationship of the spacecraft design variables and design parameters. 
\end{tabular}\\

$\Delta t_{ij}$ & 
\begin{tabular}{p{0.7\textwidth}}
Time of Flight (ToF) from node $i$ to $j$.
\end{tabular}\\

$\zeta_v$ & 
\begin{tabular}{p{0.7\textwidth}}
Propellant type for each spacecraft (predetermined). 
\end{tabular}\\

\hline
\emph{Sets} &\\
\hline
$\mathcal{A(V,N,N,T)}$ & 
\begin{tabular}{p{0.7\textwidth}}
Set of arcs realized by spacecraft.
\end{tabular}\\

$\mathcal{N}$ & 
\begin{tabular}{p{0.7\textwidth}}
Set of nodes.
\end{tabular}\\

$\mathcal{T}$ & 
\begin{tabular}{p{0.7\textwidth}}
Set of time steps.
\end{tabular}\\

$\mathcal{V}$ & 
\begin{tabular}{p{0.7\textwidth}}
Set of spacecraft (vehicles).
\end{tabular}\\

\hline\hline
\end{tabular}
\end{table}

==> Ascend 2021 Journal Revision (1)/Tables/sizing_result.tex <==
\begin{align}
\begin{aligned}
\label{sizing}
 &m_d=\sum m_{sub} = m_{str}+m_{prop}+m_{power}+m_{avi}+m_{ECLSS}+m_{misc}
    \\[0.5em] & \text { where }\\
    & \begin{array}{ll}
        \quad m_{str} &= {n_{stg}}^{-0.6705}\,(0.3238\,{m_{d}} + 693.7\,{m_{p}}^{0.04590}) 
        \\[1em]
        \quad m_{prop} &= {0.1648}\,(m_{d}+m_{p})+20.26\,\left(\dfrac{m_{f}}{\rho_{f}}\right)
        \\[1em]
        \quad m_{power} &= 7.277\cdot10^{-8}\,{m_{d}}^{2.443}+137.0
        \\[1em]
        \quad m_{avi} &= 1.014\,{m_{power}}^{0.8423}+22.33\,{t_{mis}}
        \\[1em]
        \quad m_{ECLSS} &= 0.004190\,n_{crew}\,t_{mis}\,{m_{d}}^{0.9061}\,{n_{stg}}^{0.7359}+434.7
        \\[1em]
        \quad m_{misc} &= c_{misc}\, m_{d}
    \end{array}
\end{aligned}
\end{align}

==> Eqns/MissionParameter.tex <==
\begin{table}
\caption{\label{MisisonParameter} Variables and parameters used in the space transportation scheduling problem}
\centering
\begin{tabular}{p{0.5\textwidth}p{0.15\textwidth}}
\hline Parameters & Assumption \\\hline

Spacecraft Propellant type, $zeta$ & LH2/LOx \\
Propellant $I_{sp}$, s & 420 \\
Type of Spacecraft designed  & 1 \\
Number of vehicles for each type & 6 \\
Crew mass (including space suit), kg/person & 100 \\
Crew consumption, kg/day/person & 8.655 \\
Spacecraft maintenance, structure mass/flight & 1\% \\
ISRU maintenance rate, system mass/ year & 5\% \\

\hline
\end{tabular}
\end{table}

==> Eqns/Subprob1_Def.tex <==
\begin{equation}
\label{SubSL_obj}
\min \quad \sum_{t\in \mathcal{T}} \sum_{(v,i,j)\in \mathcal{A}} (\boldsymbol{a}_{vijt}^{T} \boldsymbol{x}_{vijt} + {a'}_{vijt}^{T} m_{d_{v}} u_{vijt}) + \phi_{1}\left(\boldsymbol{c}_{1}\left(\boldsymbol{y}, \boldsymbol{y}_{1}\right)\right) 
\end{equation}

subject to
\begin{equation}
\label{SubSL_constr1}
\sum_{(v,j):(v,i,j)\in \mathcal{A}} \left[\begin{array}{c}
\boldsymbol{x}_{vijt} \\
m_{d_v}u_{vijt}
\end{array}\right] - \sum_{(v,j):(v,i,j)\in \mathcal{A}} Q_{vjit} \left[\begin{array}{c}
\boldsymbol{x}_{vji(t-\Delta t_{ji})} \\
m_{d_{v}} u_{vji(t-\Delta t_{ji})}
\end{array}\right]
\leq \boldsymbol{d}_{it} \quad \forall t\in \mathcal{T}\quad \forall i\in \mathcal{N} 
\end{equation}


\begin{equation}
\label{SubSL_constr2}
    {H}_{vij} \boldsymbol{x}_{vijt} \leq \boldsymbol{e}_v u_{vijt}  \quad \forall t\in \mathcal{T} \quad \forall (v,i,j)\in \mathcal{A}
\end{equation}

\begin{equation}
\left\{\begin{array}{ll}
\boldsymbol{x}_{vijt} \geq \boldsymbol{0}_{p \times 1}  &\text { if } t \in W_{i j} \\
\boldsymbol{x}_{vijt} =\boldsymbol{0}_{p \times 1} \quad &\text { otherwise }
\end{array} \quad \forall(v, i, j, t) \in \mathcal{A}\right.
\end{equation}

\begin{equation}
\begin{aligned}
\boldsymbol{x}_{v i j t}=\left[\begin{array}{c}
x_{1} \\
x_{2} \\
\vdots \\
x_{p}
\end{array}\right]_{v i j t}, \quad \begin{aligned}
&x_{n} \in \mathbb{R}_{\geq 0} \quad \forall n \in \mathcal{C}_{c} \\
&x_{n} \in \mathbb{Z}_{\geq 0} \quad \forall n \in \mathcal{C}_{d}
\end{aligned} \quad \forall(v, i, j, t) \in \mathcal{A} \\
\end{aligned}
\end{equation}

\begin{equation}
{u}_{v i j t} \in \mathbb{Z}_{\geq 0}  \quad \forall(v, i, j, t) \in \mathcal{A} 
\end{equation}

\begin{equation}
\boldsymbol{e}_v =  \left[\begin{array}{c}
m_{p} \\
m_{f} 
\end{array}\right]_{v}, \quad m_{p_v}, m_{f_v}, m_{d_v} \in \mathbb{R}_{\geq 0}, \quad \forall v \in \mathcal{V} 
\end{equation}

\begin{equation}
\boldsymbol{y}_1 = [m_{p_1}, m_{f_1}, m_{d_1}, \dots, m_{p_N}, m_{f_N}, m_{d_N}]
\end{equation}

==> Tables/Old&Unused/ALCresults2.tex <==
\begin{table}[h]
\caption{\label{ALCresults2} Optimization results by the decomposition-based formulation, set 2}
\centering
\begin{tabular}{cccccc}
\hline\hline
Piecewise linear   approximation step size, kg & 8000   & 4000   & 2000   & 1000   & 500    \\
\hline
Initial guess IMLEO, kg                        & 700103 & 688884 & 678633 & 677737 & 677390 \\
IMLEO, kg                                      & 694820 & 686199 & 678391 & 677542 & 677245 \\
$m_p$, kg                                         & 2882   & 2860   & 2838   & 2836   & 2834   \\
$m_f$, kg                                         & 44335  & 43627  & 42980  & 42923  & 42901  \\
$m_d$, kg                                         & 13098  & 12919  & 12757  & 12743  & 12736  \\
\hline
Initial guess generation time, s               & 5.176  & 12.19  & 3.569  & 33.22  & 1070   \\
Decomposition-based optimization time, s       & 24.23  & 19.75  & 13.30  & 13.36  & 13.97  \\
Total optimization time, s                     & 29.40  & 31.95  & 16.87  & 46.58  & 1084  \\
\hline\hline
\end{tabular}
\end{table}

==> Tables/Old&Unused/CombinedBestResults.tex <==
\begin{table}[h]
\caption{\label{CombBestRes} Best-/Worst-Case results comparison} 
\centering
\begin{tabular}{ccccc}
\hline\hline
            & \multicolumn{1}{c}{\multirow{2}{*}{Proposed formulation}} & \multicolumn{3}{c}{Embedded optimization method} \\
            \cline{3-5}
            & \multicolumn{1}{c}{}                            & Ant Colony & GA     & PSO    \\
            \hline
Best IMLEO, kg   & 676930                                          & 681302     & 728831 & 677221 \\
Optimization time, s & 16.27                                           & 45.77      & 836.6  & 793.9 \\
            \hline
Worst IMLEO, kg   & 727558                                          & inf     & inf & inf \\
Optimization time, s & 33.96                                           & 45.77      & 836.6  & 793.9 \\
\hline\hline
\end{tabular}
\end{table}

==> Tables/Old&Unused/PSOincrements.tex <==
\begin{table}
\centering
\caption{\label{PSOincrements}\new{Default instance PSO embedded optimization results with various increments}}
\begin{tabular}{cccc} 
\hline\hline
PWL increment, kg   & Algorithm & Opt.
  time, s & IMLEO, kg  \\ 
\hline
\multirow{2}{*}{10,000} & PSO       & 69.06           & 719,166    \\
                        & Proposed  & 20.02           & 724,776    \\ 
\hline
\multirow{2}{*}{5,000}  & PSO       & 67.98           & 694,224    \\
                        & Proposed  & 13.47           & 694,224    \\ 
\hline
\multirow{2}{*}{2,500}  & PSO       & 68.22           & 764,402    \\
                        & Proposed  & 10.36           & 676,862    \\ 
\hline
\multirow{2}{*}{1,250}  & PSO       & 69.00           & 677,303    \\
                        & Proposed  & 13.83           & 677,204    \\ 
\hline
\multirow{2}{*}{625}    & PSO       & 68.33           & 677,283    \\
                        & Proposed  & 13.18           & 677,072    \\
\hline\hline
\end{tabular}
\end{table}

==> Tables/Old&Unused/PSOinstances10gen.tex <==
\begin{table}
\centering
\caption{\label{PSOinstances10gen}\new{PSO embedded optimization results for all instances at 10 generations}}
\begin{tabular}{cccccc} 
\hline\hline
Instance           & Algorithm & Opt. time, s & Avg. IMLEO, kg & Best IMLEO, kg & Worst IMLEO, kg  \\ 
\hline
\multirow{2}{*}{1 (default)} & PSO       & 74.57        & 755,394        & 700,227        & inf              \\
                   & Proposed  & 11.98        & 676,862        & -              & -                \\ 
\hline
\multirow{2}{*}{2} & PSO       & 84.70        & 472,243        & 436,363        & inf              \\
                   & Proposed  & 10.70        & 401,093        & -              & -                \\ 
\hline
\multirow{2}{*}{3} & PSO       & 153.0        & 453,084        & 423,873        & inf              \\
                   & Proposed  & 61.57        & 387,535        & -              & -                \\ 
\hline
\multirow{2}{*}{4} & PSO       & 82.52        & 470,538        & 470,538        & 470,538          \\
                   & Proposed  & 22.63        & 470,406        & -              & -                \\ 
\hline
\multirow{2}{*}{5} & PSO       & 75.36        & 460,932        & 451,269        & 470,869          \\
                   & Proposed  & 94.06        & 442,605        & -              & -                \\ 
\hline
\multirow{2}{*}{6} & PSO       & 96.64        & 320,680        & 305,457        & 337,105          \\
                   & Proposed  & 14.30        & 293,095        & -              & -                \\ 
\hline
\multirow{2}{*}{7} & PSO       & 172.3        & 322,115        & 302,791        & 358,768          \\
                   & Proposed  & 44.02        & 302,041        & -              & -                \\ 
\hline
\multirow{2}{*}{8} & PSO       & 94.21        & 372,485        & 355,767        & 395,748          \\
                   & Proposed  & 14.47        & 344,423        & -              & -                \\
\hline\hline
\end{tabular}
\end{table}

==> Tables/Old&Unused/basecase_comparison.tex <==
\begin{table}
\caption{\label{BasecaseComparison} \textcolor{red}{Default instance average results by the embedded optimization over 10 iterations}}
\centering
\begin{tabular}{cccc}
\hline\hline
Algorithm & Number of generations & Optimization time, s & IMLEO, kg  \\ 
\hline
          & 10                    & 72.27                & 782,304    \\
ACO       & 50                    & 360.9                & 742,573    \\
          & 100                   & 721.2                & 718,586    \\ 
\hline
          & 10                    & 80.58                & 822,926    \\
GA        & 50                    & 413.1                & 770,917    \\
          & 100                   & 814.8                & 752,836    \\ 
\hline
          & 10                    & 74.57                & 755,394    \\
PSO       & 50                    & 381.7                & 702,581    \\
          & 100                   & 765.3                & 691,196    \\ 
\hline
Proposed  & -                   & 10.36                & 676,862    \\
\hline\hline
\end{tabular}
\end{table}

==> Tables/Old&Unused/embedded_highlight.tex <==
\begin{table}[h]
\caption{\label{EmbeddedHighlight} Results of the state-of-the-art embedded optimization}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccccc}
\hline\hline
% \multicolumn{1}{c}{Algorithm} & \multicolumn{1}{c}{Number of generations} & Optimization Time, s & Best IMLEO, kg  \\
% \hline
% \multirow{3}{*}{Ant Colony Optimization}    
%      & 10  & 85.03    & 723090 \\
%      & 50   & 391.7    & 747398 \\
%      & 100 & 776.0      & 689287 \\
% \hline
% \multirow{3}{*}{Genetic Algorithm}           
%      & 10  & 86.18    & 764301 \\
%      & 50  & 413.6    & 746702 \\
%      & 100 & 836.6    & 728831 \\
% \hline
% \multirow{3}{*}{Particle Swarm Optimization} 
%      & 10 & 84.69    & inf    \\                              
%      & 50  & 397.9    & 677659 \\
%      & 100 & 793.9    & 677221 \\ 
%      \hline\hline
     
     
     
\multicolumn{1}{c}{Algorithm} & \multicolumn{3}{c}{Ant Colony Optimization} & \multicolumn{3}{c}{Genetic Algorithm} & \multicolumn{3}{c}{Particle Swarm Optimization} \\
\hline
Number of generations & 10 & 50 & 100 & 10 & 50 & 100 & 10 & 50 & 100 \\
Best Solution IMLEO, kg  & 723,090  & 747,398& 689,287 & 764,301& 746,702 & 728,831 & inf & 677,659& 677,221\\
Optimization Time, s &85.03& 391.7  & 776.0  & 86.18 & 413.6 & 836.6 & 84.69 & 397.9 & 793.9\\
\hline\hline 
\end{tabular}}
\end{table}

==> Tables/Old&Unused/embedded_highlight2.tex <==
\begin{table}[h]
\caption{\label{EmbeddedFullTable2} Summary of the embedded optimization results}
\centering
\centering
\resizebox{0.75\textwidth}{!}{%
\begin{tabular}{cccc}
\hline\hline
\multicolumn{1}{c}{Algorithm}                        & \multicolumn{1}{l}{Number of generations} & Optimization time, s & IMLEO, kg  \\
\hline
\multirow{15}{*}{Ant Colony Optimization}    
     & \multirow{3}{*}{5}                                    & 45.35    & 820891 \\
     &                                                       & 45.06    & inf    \\
     &                                                       & 45.77    & 681302 \\
     \cline{2-4}
     & \multirow{3}{*}{10}                                     & 83.19    & 806153 \\
     &                                                     & 85.03    & 723090 \\
     &                                                      & 83.81    & 793031 \\\cline{2-4}
     & \multirow{3}{*}{20}                                       & 161.4    & 714202 \\
     &                                                           & 161.2    & 801618 \\
     &                                                           & 162.3    & 710166 \\\cline{2-4}
     & \multirow{3}{*}{50}                                      & 389.8    & 761514 \\
     &                                                          & 391.2    & 765182 \\
     &                                                          & 391.7    & 747398 \\\cline{2-4}
     & \multirow{3}{*}{100}                                    & 776.0      & 689287 \\
     &                                                          & 771.9    & 732297 \\
     &                                                        & 775.9    & 691874 \\
\hline
\multirow{15}{*}{Genetic Algorithm}           
     & \multirow{3}{*}{5}                                      & 46.50     & inf    \\
     &                                                         & 45.71    & inf    \\
     &                                                        & 46.09    & inf    \\\cline{2-4}
     & \multirow{3}{*}{10}                                     & 85.38    & inf    \\
     &                                                      & 86.18    & 764301 \\
     &                                                      & 83.97    & inf    \\\cline{2-4}
     & \multirow{3}{*}{20}                                   & 161.9    & inf    \\
     &                                                        & 172.4    & 761116 \\
     &                                                       & 161.7    & inf    \\\cline{2-4}
     & \multirow{3}{*}{50}                                    & 394.7    & inf    \\
     &                                                       & 413.6    & 746702 \\
     &                                                          & 394.6    & inf    \\\cline{2-4}
     & \multirow{3}{*}{100}                                   & 836.6    & 728831 \\
     &                                                        & 788.3    & 875069 \\
     &                                                         & 777.7    & inf    \\
\hline
\multirow{15}{*}{Particle Swarm Optimization} 
     & \multirow{3}{*}{5}                                      & 46.54    & inf    \\
     &                                                         & 46.57    & inf    \\
     &                                                       & 46.26    & 711382 \\\cline{2-4}
     & \multirow{3}{*}{10}                                    & 84.75    & inf    \\
     &                                                        & 84.69    & inf    \\
     &                                                       & 85.22    & inf    \\\cline{2-4}
     & \multirow{3}{*}{20}                                     & 162.5    & 726951 \\
     &                                                       & 162.1    & 688182 \\
     &                                                         & 161.6    & inf    \\\cline{2-4}
     & \multirow{3}{*}{50}                                     & 392.3    & inf    \\
     &                                                       & 397.9    & 677659 \\
     &                                                         & 394.6    & 714169 \\\cline{2-4}
     & \multirow{3}{*}{100}                                   & 788.9    & 677754 \\
     &                                                         & 793.9    & 677221 \\
     &                                                        & 791.2    & 677316 \\
     \hline\hline
\end{tabular}}
\end{table}

==> Tables/Old&Unused/heuristics_results.tex <==
\begin{table}[h]
\caption{\label{EmbeddedFullTable} Summary of the embedded optimization results}
\centering
\resizebox{0.67\textwidth}{!}{%
\begin{tabular}{ccccc}
\hline\hline
\multicolumn{1}{c}{Algorithm}                        & \multicolumn{1}{l}{Number of Generations} & Iteration Number & Run Time, s & IMLEO, kg  \\
\hline
\multirow{15}{*}{Ant Colony Optimization}    & \multirow{3}{*}{5}                        & 1                & 45.35    & 820891 \\
                                                     &                                           & 2                & 45.06    & inf    \\
                                                     &                                           & 3                & 45.77    & 681302 \\
                                                     \cline{2-5}
                                                     & \multirow{3}{*}{10}                       & 1                & 83.19    & 806153 \\
                                                     &                                           & 2                & 85.03    & 723090 \\
                                                     &                                           & 3                & 83.81    & 793031 \\\cline{2-5}
                                                     & \multirow{3}{*}{20}                       & 1                & 161.4    & 714202 \\
                                                     &                                           & 2                & 161.2    & 801618 \\
                                                     &                                           & 3                & 162.3    & 710166 \\\cline{2-5}
                                                     & \multirow{3}{*}{50}                       & 1                & 389.8    & 761514 \\
                                                     &                                           & 2                & 391.2    & 765182 \\
                                                     &                                           & 3                & 391.7    & 747398 \\\cline{2-5}
                                                     & \multirow{3}{*}{100}                      & 1                & 776.0      & 689287 \\
                                                     &                                           & 2                & 771.9    & 732297 \\
                                                     &                                           & 3                & 775.9    & 691874 \\
\hline
\multirow{15}{*}{Genetic Algorithm}           & \multirow{3}{*}{5}                        & 1                & 46.50     & inf    \\
                                                     &                                           & 2                & 45.71    & inf    \\
                                                     &                                           & 3                & 46.09    & inf    \\\cline{2-5}
                                                     & \multirow{3}{*}{10}                       & 1                & 85.38    & inf    \\
                                                     &                                           & 2                & 86.18    & 764301 \\
                                                     &                                           & 3                & 83.97    & inf    \\\cline{2-5}
                                                     & \multirow{3}{*}{20}                       & 1                & 161.9    & inf    \\
                                                     &                                           & 2                & 172.4    & 761116 \\
                                                     &                                           & 3                & 161.7    & inf    \\\cline{2-5}
                                                     & \multirow{3}{*}{50}                       & 1                & 394.7    & inf    \\
                                                     &                                           & 2                & 413.6    & 746702 \\
                                                     &                                           & 3                & 394.6    & inf    \\\cline{2-5}
                                                     & \multirow{3}{*}{100}                      & 1                & 836.6    & 728831 \\
                                                     &                                           & 2                & 788.3    & 875069 \\
                                                     &                                           & 3                & 777.7    & inf    \\
\hline
\multirow{15}{*}{Particle Swarm Optimization} & \multirow{3}{*}{5}                        & 1                & 46.54    & inf    \\
                                                     &                                           & 2                & 46.57    & inf    \\
                                                     &                                           & 3                & 46.26    & 711382 \\\cline{2-5}
                                                     & \multirow{3}{*}{10}                       & 1                & 84.75    & inf    \\
                                                     &                                           & 2                & 84.69    & inf    \\
                                                     &                                           & 3                & 85.22    & inf    \\\cline{2-5}
                                                     & \multirow{3}{*}{20}                       & 1                & 162.5    & 726951 \\
                                                     &                                           & 2                & 162.1    & 688182 \\
                                                     &                                           & 3                & 161.6    & inf    \\\cline{2-5}
                                                     & \multirow{3}{*}{50}                       & 1                & 392.3    & inf    \\
                                                     &                                           & 2                & 397.9    & 677659 \\
                                                     &                                           & 3                & 394.6    & 714169 \\\cline{2-5}
                                                     & \multirow{3}{*}{100}                      & 1                & 788.9    & 677754 \\
                                                     &                                           & 2                & 793.9    & 677221 \\
                                                     &                                           & 3                & 791.2    & 677316\\\hline\hline
\end{tabular}}
\end{table}
